Semi-polarized meromorphic Hitchin and Calabi-Yau integrable systems

It was shown by Diaconescu, Donagi and Pantev that Hitchin systems of type ADE are isomorphic to certain Calabi-Yau integrable systems. In this paper, we prove an analogous result in the setting of meromorphic Hitchin systems of type A which are known to be Poisson integrable systems. We consider a symplectization of the meromorphic Hitchin integrable system, which is a semi-polarized integrable system in the sense of Kontsevich and Soibelman. On the Hitchin side, we show that the moduli space of unordered diagonally framed Higgs bundles forms an integrable system in this sense and recovers the meromorphic Hitchin system as the fiberwise compact quotient. Then we construct a new family of quasi-projective Calabi-Yau threefolds and show that its relative intermediate Jacobian fibration, as semi-polarized integrable systems, is isomorphic to the moduli space of unordered diagonally framed Higgs bundles.

==> CYintegrable.tex <==

    
\subsection{Construction}
In this section, we shall generalize Smith's elementary modification idea \cite{smith2015quiver} to construct a (semi-polarized) Calabi-Yau integrable system. A similar construction is also used in the work of Abrikosov \cite[Section 6]{abrikosov2018potentials} and Smith \cite{smith2020floer}.
 
First, we describe the construction of a family of Calabi-Yau threefolds. Let $V:= \Tot(K_{\sm}(D)\oplus (K_{\sm}(D))^{n-1}\oplus K_{\sm}(D)) $ and consider the short exact sequence
        \begin{equation*}
            0\to \cO_{\sm}(-D)\xrightarrow{\alpha} \cO_{\sm}\to i_{D*}\cO_D \to 0.
        \end{equation*}
        where we recall $i_D:D \hookrightarrow X$ is the natural inclusion. Suppose $u$ is a local frame of $\cO_{\sm}(-D)$. In terms of a local coordinate $z$ around a point of $D$ where $z=0$, $\alpha(u)$ is represented by $f\cdot u$ where $f$ is a locally defined function that vanishes at $z=0.$ 
        We define an elementary modification $\wv$ of $V$ along the first component: 
        \begin{equation*}
             \wv :=\Tot (K_{\sm}(D-D)\oplus (K_{\sm}(D))^{n-1}\oplus K_{\sm}(D))\to \Tot(K_{\sm}(D)\oplus (K_{\sm}(D))^{n-1}\oplus K_{\sm}(D)) 
        \end{equation*}
        and denote the projection map by $\wpi: \wv\to \sm.$ 
        
        For $b =(b_2(z),...,b_n(z)) \in B= \oplus_{i=2}^n H^0({\sm}, K_{\sm}(D)^{\otimes i})$, we define the threefold $X_b$ as the zero locus of a section in $\Gamma(\wv, \wpi^*K_{\sm}(D)^{\otimes n})$:
        \begin{equation} \label{defining equation}
            X_b:= \{\alpha(x)y - s^n  -\wpi^*b_2(z) s^{n-2} -... -\wpi^*b_n(z) =0 \}\subset \wv
        \end{equation}
        with the projection $\pi_b:X_b \to \Sigma$. Here we denote by $x, y$ and $s$ the tautological sections of the pullback of $K_\sm,(K_\sm(D))^{n-1}$ and $K_\sm(D)$, respectively.
        Note that each term in the equation (\ref{defining equation}) is a section of $\wpi^*K_{\sm}(D)^{\otimes n}$. More explicitly, we have
        \begin{align*}
            &x\in \Gamma ( \wv, \wpi^*K_{\sm}), \quad \alpha(x) \in \Gamma (\wv, \wpi^*K_{\sm}(D)), \quad 
             y\in \Gamma ( \wv, \wpi^*(K_{\sm}(D))^{n-1})\\ &
            s\in \Gamma ( \wv, \wpi^*K_{\sm}(D)),\quad  \pi^*b_i \in \Gamma (\wv,\wpi^*(K_{\sm}(D))^i) 
        \end{align*}
        This construction gives rise to a family of quasi-projective threefolds 
        \begin{equation*}
             pr_2 \circ \bm{\pi}:\cX \to B.
        \end{equation*}
        
        Next, we show that the threefold $X_b$ is indeed a non-singular Calabi-Yau threefold.
        \begin{prop}
        The threefold $X_b$ has trivial canonical bundle.
        \end{prop}
        \begin{proof}
           By the adjunction formula, 
        \begin{equation*}
            K_{X_b} = K_{\wv} \otimes \wpi^* (K_{\sm}(D))^{\otimes n}|_{X_b}.
        \end{equation*}
        where $\wpi: \wv\to {\sm}.$ Note that 
        \begin{equation*}
            K_{\wv} = \wpi^*\det ( \wv^\vee ) \otimes \wpi^*K_{\sm} \cong \wpi^*(K_{\sm}^{-n-1}(-nD)) \otimes \wpi^*K_{\sm} \cong \wpi^*(K_{\sm}^{-n}(-nD)).
        \end{equation*}
        So it follows that 
        \begin{equation*}
            K_{X_b} = \wpi^*(K_{\sm}^{-n}(-nD)) \otimes \wpi^* (K_{\sm}(D))^{\otimes n}|_{X_b} \cong \cO_{X_b}.
        \end{equation*}
        \end{proof}
    \begin{prop}
       For each $b\in B^{ur}$, the threefold $X_b$ is non-singular. 
    \end{prop}
    \begin{proof}
            This is a local statement, so we can restrict to neighbourhoods in $\sm.$ 
            Around a point of $D$ with local coordinate $z$, the local model of $X_b$ is 
            \begin{equation*}
                \{f(z) xy - s^n  -\widetilde{b}_2(z) s^{n-2} -... -\widetilde{b}_n(z) =0 \}\subset \C^3_{(x,y,s)} \times \C_z,
            \end{equation*}
            where $\widetilde{b}_i$ are now functions of $z$, and $f(z)$ is function with zero only at $z=0.$ We check smoothness by examining the Jacobian criterion. The equation
            \begin{equation}\label{spectral_cover_equation}
                \frac{\partial}{\partial s} \big(s^n  -\widetilde{b}_2(z) s^{n-2} -... -\widetilde{b}_n(z) \big ) = 0
            \end{equation}
            implies that, for each $z$, the equation $s^n  -\widetilde{b}_2(z) s^{n-2} -... -\widetilde{b}_n(z)=0$ must have repeated solutions, this happens only when $z$ is at the branch locus of the spectral curve associated to $b$. The remaining equations in the Jacobian criterion are
            \begin{equation*}
                f(z) y= 0, \quad f(z)x =0 , \quad f'(z) xy +\frac{\partial}{\partial z}\big(s^n  -\widetilde{b}_2(z) s^{n-2} -... -\widetilde{b}_n(z)\big)=0
            \end{equation*}
            When $x=y=0$, the equation $\frac{\partial}{\partial z}\big(s^n  -\widetilde{b}_2(z) s^{n-2} -... -\widetilde{b}_n(z)\big)=0$ has no solution since we assume that the spectral curve associated to $b$ is smooth and equation (\ref{spectral_cover_equation}) has a solution. Hence, it must be the case that $x\neq 0$ or $y\neq 0$ which implies that $f(z)=0$ or equivalently $z=0$. However, since we assume $b\in B^{ur}$ which means that the spectral curve must be unramified over $D$, this is a contradition and so $X_b$ is non-singular around $D.$ 
            
            Away from $D$, a similar argument shows that the threefold is non-singular over the local neighbourhood. Hence, $X_b$ is non-singular everywhere. 
            
    \end{proof}
    Again, by examining the defining equation (\ref{defining equation}), we can list the types of fibers of the map $\pi_b:X_b \to \sm$: 
    \begin{itemize}
        \item For $p\in D$ with coordinate $z=0$, the fiber is defined by the equation \\ $s^n  -\widetilde{b}_2(z) s^{n-2} -... -\widetilde{b}_n(z)=0$, i.e. disjoint union of $n$ copies of $\C^2.$ 
        \item For a critical value $p$ of $\pi_b$, the fiber is defined by $xy - \prod_{i=1}^m(s-s_i)^{k_i} $ where $\sum_{i=1}^m k_i = n$ $(m<n)$. Hence, the fiber is a singular surface with $A_{k_i-1}$-singularity at $s_i$. 
        \item For $p$ away from $D$ and the discriminant locus of $\pi_b$, the fiber is defined by $(xy -s^n ) -\widetilde{b}_2(z) s^{n-2} -... -\widetilde{b}_n(z)= 0$ and smooth, so it is isomorphic to a smooth fiber of the universal unfolding of $A_{n-1}$-singularity $\C^2/\Z_n$.  
    \end{itemize}
    \todo{Start new chapter:Gluing and prove that $\cY^\circ \cong \cX^\circ$}\\
    \todo{Next, prove mHS result and talk about semi-polarized integrable system}
    
    We are particularly interested in $\Z$-mixed Hodge structures on the third (co)homology group of $X_b$. Let's denote the complement of $\pi_b^{-1}(D)$ by $X_b^\circ$.

    \begin{lem}\label{lem:puncture iso}
    For $b \in B^{ur}$, there are isomorphisms of $\Z$-mixed Hodge structures
    \begin{equation}
        \begin{aligned}
        H_3(X_b, \Z)(-3) \cong H_c^3(X_b, \Z) \cong H_c^3(X_b^\circ, \Z), \quad H^3(X_b, \Z) \cong H^3(X_b^\circ, \Z)
        \end{aligned}
    \end{equation}
    \end{lem}
    \begin{proof}
        It is enough to show that $H_c^3(X_b, \Z) \cong H_c^3(X_b^\circ, \Z)$ since the other isomorphisms follow from the Poincar\'e duality. Consider the long exact sequence of compactly supported cohomologies associated to the pair $(X_b, \pi_b^{-1}(D))$
        \begin{equation*}
        \cdots \to H_c^2(\pi^{-1}_b(D),\Z) \to H_c^3(X_b^\circ,\Z) \to H_c^3(X_b,\Z) \to H_c^3(\pi^{-1}_b(D),\Z) \to \cdots
    \end{equation*}
    As $H_c^2(\pi^{-1}_b(D),\Z)=H_c^3(\pi^{-1}_b(D),\Z)=0$, we have an isomorphism of $\Z$-mixed Hodge structures
    \begin{equation} \label{eq:3 cohomology equal compactly supported}
        H^3_c(X_b,\Z) \cong H^3_c(X_b^\circ,\Z)
    \end{equation}
    \end{proof} 
    
    Now, we focus on the $\Z$-mixed Hodge structures of $H_3(X_b^\circ,\Z)$ and $H^3(X_b^\circ, \Z)$. 
      
    \begin{prop}\label{Hodge type argument}
        For $b \in B^{ur}$, the third homology group $H_3(X_b,\Z)$ admits a $\Z$-mixed Hodge structure of
        type  $\{(-2,-2),(-2,-1),(-1,-2)\}$. Moreover, the third cohomology group $H^3(X_b,\Z)$ admits a $\Z$-mixed Hodge structure of type $\{(1,2),(2,1),(2,2)\}$.
    \end{prop}
    
    \begin{proof}
    
        By Lemma \ref{lem:puncture iso} and Poincar\'e duality, we only need to show that the third compactly supported cohomology group $H_c^3(X_b^\circ,\Z)$ admits a $\Z$-mixed Hodge structure of type $\{(1,1),(1,2),(2,1)\}$. We mainly follow the approach in \cite[Lemma 3.1]{diaconescu2006intermediate}. As we are mainly interested in Hodge type, we work over the coefficient $\C$, instead of $\Z$. We drop the subscript $b$ for simplicity. Let $\pi^\circ: = \pi|_{\sm^\circ}$ and $\crit(\pi^\circ) \subset X^\circ$ be the finite set of critical values. We write $(-)_{reg}$ for a regular part of a given space. In other words, we have the following commutative diagram of non-singular varieties
        \begin{equation*}
            \begin{tikzcd}
            X^\circ_{reg}:= (\pi^\circ)^{-1}({\Sigma^\circ_{reg}}) \arrow[r, hook] \arrow[d, "\pi_{reg}^\circ"]& X^\circ \arrow[d, "\pi^\circ"] \arrow[r, hook]& X \arrow[d, "\pi"] 
            \\
            \Sigma^\circ_{reg}:=\Sigma^\circ \setminus \crit(\pi^\circ) \arrow[r, hook,  "j_{reg}"] & \Sigma^\circ \arrow[r, hook, "j"] & \sm
            \end{tikzcd}
        \end{equation*}
        
        
         We apply the Leray spectral sequence associated to $\pi^\circ:X^\circ \to \Sigma^\circ$, whose $E_2$-page is given by
        \begin{equation}
            E_2^{pq}=H_c^p(\Sigma^\circ, R^q\pi^\circ_!\C)
        \end{equation}
        We first claim that only $E_2^{12}$-term does not vanish so that $E_2^{12}= H^1_c(\sm^\circ, R^2\pi_!^\circ \C) \cong E_{\infty}^{12}=H_c^3(X^\circ, \C)$. This follows from the topology of each fiber of $\pi^\circ$. For $z \in \sm^\circ_{reg}$, a fiber of $(\pi^\circ)^{-1}(z)$ is deformation equivalent to a smooth fiber of the universal unfolding of $A_{n-1}$-singularity $\C^2/\Z_n$ whose (compactly supported) cohomology is given by 
         \begin{equation*}
            H^*((\pi^\circ)^{-1}(z), \C)=\begin{cases}
            \C & *=0 \\
            \C^{n} & *=2 \\
            0 & * \neq 0,2
            \end{cases}
         \end{equation*}
        For $z \in \crit(\pi^\circ)$, since we restrict that $b \in B^{ur}$, the singular fibers of $\pi^\circ$ have a single node and is isomorphic to a smooth fiber of the universal unfolding of $A_{n-1}$-singularity $\C^2/\Z_n$ with a $(-2)$-curve contracted, hence only $R^2\pi^\circ_!\C$ is non-vanishing. Furthermore, one can see that the natural morphism $R^2\pi_!\C \to R^2\pi_*\C$ \todo{circle?} is an isomorphism. 
        
        \todo{JC:} \\
        In section 4.2, we will show that there exists a smooth threefold $Y$ (depending on $b$)\footnote{In section 4.2, $Y$ is constructed as the member of the family $\cY^{ur}$ over $b\in B^{ur}$.} with a morphism $\pi_Y: Y\to \sm$ such that if we denote by $Y^\circ:= Y|_{\sm^\circ}$ and $\pi_Y^\circ:= (\pi_Y)|_{\sm^\circ}$, Lemma \ref{gluingmodel} says that $Y^\circ\cong X^\circ$ and $\pi_Y^\circ \cong \pi^\circ$. In fact, the threefold $Y$ is exactly the smooth non-compact Calabi-Yau threefold used in \cite[Lemma 3.1]{diaconescu2006intermediate}. So, if we write $\overline{\cF}:= R^2\pi_{Y!} \C $, we have $j^*\overline{\cF} \cong R^2\pi^\circ_!\C$. By applying the following exact triangle in the derived category $D^b_c(\sm)$ of constructible sheaves on $\sm$ to $\overline{\cF}$ 
         \begin{equation*}
             j_!j^* \to id \to i_*i^* \xrightarrow{+1}
         \end{equation*}
         we obtain a long exact sequence of mixed Hodge structures,  
        \begin{equation*}
                H^0(\sm, \overline{\cF}) \xrightarrow{\phi} H^0(D, \overline{\cF}|_D) \to H_c^1(\sm^\circ, R^2\pi^\circ_!\C) \to H^1(\sm, \overline{\cF}) \to 0
            \end{equation*}
        Note that the morphism $\phi$ is not surjective when $|D|\geq 2$. Then, as argued in \cite[Lemma 3.1]{diaconescu2006intermediate}, the term $H^1(\sm, \overline{\cF})$ has a pure Hodge structure of type $\{(1,2),(2,1)\}$. Also, in \textit{loc.cit.}, it is argued that for the fiber $Y_t$ of $Y$ over each $t\in D$, $H^2(Y_t,\C)$ is pure of type $(1,1)$ and so is $H^2_c(Y_t,\C)$. Hence, $H^0(D, \overline{\cF}|_D)$ is pure of type $(1,1)$ and we can conclude that the $\Z$-mixed Hodge structure on $H^3_c(X^\circ,\Z)\cong H^1_c(\sm^\circ, R^2\pi^\circ_!\C)$ is of type $\{(1,1),(1,2),(2,1)\}$. 
        
        
        % Next, we consider the natural adjunction $R^2\pi_{!(*)}^\circ\C \to j_{reg*}j_{reg}^*R^2\pi_{!(*)}^\circ\C$ \todo{what is $!(*)?$} \todo{just say $R^2\pi_{!}^\circ\C \to j_{reg*}j_{reg}^*R^2\pi_{!}^\circ\C$ (respectively $R^2\pi_{*}^\circ\C \to j_{reg*}j_{reg}^*R^2\pi_{*}^\circ\C$)?} \todo{you trying to show $R^2\pi^\circ_{!}\C \to j_*j^*R^2\pi^\circ_!\C$ right?} and show that it is an isomorphism. One can directly show this by computing the monodromy around the singular fibers \todo{fibers over $D$?}. Instead, we refer to the result in \cite[Section 3.5]{beck2017hitchin} to make a connection with the proof of Theorem \ref{thm:main meromorphic DDP}. To apply this result, the gluing structure of $X^\circ$ is crucial, which we study in the next section (see Section \ref{sec:CYIS}). More precisely, there is a fibration on a smooth threefold $Y$ (depending on $b \in B^{ur}$), $\pi_Y:Y \to \sm$ such that it is locally trivial  over \todo{smooth} $D \subset \sm$ and the restriction over the complement of $(\pi_Y)^{-1}(D)$, denoted by $Y^\circ$, is isomorphic to $\pi^\circ: X^\circ \to \sm^\circ$. It implies that the monodromy of $j_{reg*}R^2\pi^\circ_{reg!(*)}\C$ \todo{same here} on $\sm^\circ$ around $D$ is trivial. For simplicity, we set $\cF:=R^2\pi^\circ_{reg!(*)}\C$ \todo{same here} and $\bar{\cF}$ to be the trivial extension such that $j^*\bar{\cF}=j_{reg*}\cF$. 
        
        
        
        
        % By applying $\bar{\cF}$ to the following exact triangle on the derived category $D^b_c(\sm)$ of constructible sheaves on $\sm$ \todo{apply to $\overline{\cF}$?}
        %  \begin{equation*}
        %      j_!j^* \to id \to i_*i^* \xrightarrow{+1}
        %  \end{equation*}
        %  we obtain a long exact sequence of mixed Hodge structures, 
        %  \begin{equation*}
        %         H^0(\sm, j_*j_{reg*}\cF) \xrightarrow{\phi} H^0(D, \cF_0) \to H_c^1(\sm^\circ, j_{reg*}\cF) \to H^1(\sm, j_*j_{reg*}\cF) \to 0
        %     \end{equation*}
        %     \todo{$j_*j_{reg_*}$}
        % where $\cF_0$ is a stalk of $\cF$ over a generic point. The last term admits a pure Hodge structure of type $\{(1,2),(2,1)\}$ by Zucker's theorem \cite{Zucker} \todo{since }. Also, one can see that the morphism $\phi$ is not surjective because $|D| \geq 2$ and $H^0(D, \cF_0)$ admits a Hodge structure of type $(1,1)$. Therefore, we conclude that the $\Z$-mixed Hodge structure on $H^3_c(X^\circ, \Z)$ is of type $\{(1,1), (1,2), (2,1)\}$. 
        
    \end{proof}
    
    By taking a Tate twist by $-1$, we have the $\Z$-mixed Hodge structure $H_3(X_b, \Z)(-1)$ of type $\{(-1,-1), (-1,0), (0,-1)\}$. The homology version of the second intermediate Jacobian of $X_b$ is defined to be the Jacobian associated to the $\Z$-mixed Hodge structure $H_3(X_b,\Z)(-1)$
    \begin{equation}
        J_2(X_b):=J(H_3(X_b,\Z)(-1))=\frac{H_3(X_b,\C)(-1)}{F^{-1}H_3(X_b,\C)(-1)+H_3(X_b,\Z)(-1)}
    \end{equation}
    
    \begin{rem}
    The third homology group $H_3(X_b,\Z)$  turns out to have a torsion (see Theorem \ref{localDDP}). To get the $\Z$-mixed Hodge structure on the lattice of the semi-abelian variety $J_2(X_b)$, we should consider the $\Z$-mixed Hodge structure on the torsion-free part $H_3(X_b,\Z)_{\textrm{tf}}$.
    \end{rem}
    
    \begin{cor}
    For $b \in B^{ur}$, the homology version of the second intermediate Jacobian $J_2(X_b)$ is a semi-abelian variety. 
    \end{cor}
    
    \begin{rem}(Adjoint Type)\label{rem:CYadjointtype}
    Unlike the holomorphic case in \cite{diaconescu2006intermediate}, the cohomological intermediate Jacobian on $H^3(X_b,\Z)$ is not a semi-abelian variety because of the Hodge type (see Appendix \ref{appendix}). This is one of the new features, so we need to consider different data to describe the case of  $PGL(n,\C)$, the adjoint group of type A. It turns out that the right object is a mixture of compactly supported cohomology and ordinary cohomology associated to $\pi_b:X_b \to \Sigma$:
    \begin{equation*}
        H^1_c(\sm,R^2\pi_{b*}\Z)\cong H^1_c(\sm^\circ,R^2\pi^\circ_{b*}\Z).
    \end{equation*}
    which can be considered a different integral structure on $H_c^3(X_b, \C)$.
    \end{rem}
    
    \subsection{Calabi-Yau integrable systems} \label{sec:CYIS}
    Having constructed the family of Calabi-Yau threefolds $\cX^{ur}\to B^{ur}$, we can consider the relative intermediate Jacobian fibration $\pi^{ur}:\cJ(\cX^{ur}/B^{ur}) \to B^{ur}$ whose fiber is $J_2(X_b)= H_3(X_b,\C) /(F^{-1}H_3(X_b,\C)+ H_3(X_b,\Z))$. One way to equip it with an integrable system structure is to find an abstract Seiberg-Witten differential (see Section 2). In the case of an intermediate Jacobian fibration, this can be achieved by finding a global nowhere-vanishing holomorphic volume form in each fiber. The resulting semi-polarized integrable system will again be called the Calabi-Yau integrable system.
    
    Consider the subfamily of Calabi-Yau threefolds
    \begin{equation*}
        (\cX^\circ)^{ur}: = \cX^{ur} \setminus \bm{\pi}^{-1}(D\times B^{ur}) \subset \cX^{ur} \to B^{ur}.
    \end{equation*}
    whose fiber is $X_b^\circ:= X_b \setminus \pi_b^{-1}(D)$. From the relation (\ref{eq:3 cohomology equal compactly supported}), it is enough to find global holomorphic volume forms for the family $(\cX^\circ)^{ur}\to B^{ur}$. The idea is that the family $(\cX^\circ)^{ur}\to B^{ur}$ can be constructed alternatively by gluing Slodowy slices as in  \cite{diaconescu2006intermediate}\cite{beck2017hitchin}, which is the key ingredient used for the existence of global volume forms.

    


\begin{claim}\label{gluing of slodowy}
The family of quasi-projective Calabi-Yau threefolds $\pi^{ur}:(\cX^\circ)^{ur} \to B^{ur}$ can be obtained by gluing Slodowy slices. 
\end{claim}

Recall that in the classical case \cite{slodowy1980four}, the Slodowy slice $S\subset \fg$ provides a semi-universal $\C^*$-deformation $\sigma:S\to \ft /W$ of simple singularities via the adjoint map $\sigma:\fg\to \ft/W$. However, if we denote by $d_j$ the standard ($\C^*$-action) weights of the generators of the coordinate ring $\C[\chi_1,...,\chi_j]$ of $\ft/W$, then the weights on $\C[\chi_1,...,\chi_j]$ must be chosen as $2d_j$ for $\sigma$ to be $\C^*$-equivariant (see \cite[Remark 2.5.3]{beck2020folding}, \cite{slodowy1980four}). 

Now we choose a theta characteristic $L$ on $\sm$, i.e. $L^2 \cong K_\sm$. Since $L^2|_{\sm^\circ}\cong K_{\sm}|_{\sm^\circ}\cong K_{\sm}(D)|_{\sm^\circ}$, we have an isomorphism of associated bundles over $\sm^\circ$
\begin{equation*}
    L|_{\sm^\circ}\times_{\C^*} \ft/W \cong  K_{\sm}(D)|_{\sm^\circ}\times_{\C^*} \ft/W
\end{equation*}
where the weights of the $\C^*$-action on both sides are different: the left hand side has weights $2d_j$ and the right hand side has weights $d_j.$ As the map $\sigma:S\to \ft/W$ is $\C^*$-equivariant, we can glue it along $\Tot(L)$ to obtain 
\begin{equation*}
    \bm{\sigma} : \bm{S}: = \Tot (L\times _{\C^*}S) \to \Tot(L\times_{\C^*} \ft/W)
\end{equation*}
and its restriction
\begin{equation*}
    \bm{\sigma}|_{\sm^\circ} : \bm{S}|_{\sm^\circ}: = \Tot (L\times _{\C^*}S)|_{\sm^\circ} \to \Tot(L|_{\sm^\circ}\times_{\C^*} \ft/W)\cong \Tot(K_\sm(D)|_{\sm^\circ}\times_{\C^*}\ft/W) = \bm{U}|_{\sm^\circ} .
\end{equation*}
Pulling back under the evaluation map from $\Sigma \times B$, one gets the two families of quasi-projective threefolds $\cY^{ur}$ and $(\cY^\circ)^{ur}$ as follows:
\begin{equation}\label{CYfamilies}
\begin{tikzcd}
    \cY^{ur} \arrow[r] \arrow[d, "\pi'"] & \bm{S} \arrow[d, "\bm{\sigma}"] \\
    \Sigma \times B^{ur} \arrow[r, "ev"] & \bm{U}
    \end{tikzcd},\quad 
    \begin{tikzcd}
    (\cY^\circ)^{ur} \arrow[r] \arrow[d, "\pi'"] & \bm{S}|_{\sm^\circ} \arrow[d, "\bm{\sigma}|_{\sm^\circ}"] \\
    \Sigma^\circ \times B^{ur} \arrow[r, "ev"] & \bm{U}|_{\sm^\circ}
    \end{tikzcd}
\end{equation}
Clearly, the restriction of $\cY^{ur}$ over $\sm^\circ \times B^{ur}\subset B^{ur}$ is $(\cY^\circ)^{ur}$. 
\todo{addded another family}

%Given a line bundle $K_\Sigma(D)$, one can glue those Slodowy slices over $\Tot(K_\Sigma(D))$ with respect to its $\C^*$-action. Pulling back under the evaluation map from $\Sigma \times B$, one gets a family of quasi-projective threefolds $\cX'$ as follows:

%However, a generic fiber of $\pi'|_B:\cX' \to B$ is not Calabi-Yau because the anti-canonical divisor is linearly equivalent to the preimage of the divisor $D$, $(\pi')^{-1}_b(D) \subset X_b$. A trick is to remove the fiber $(\pi'_b)^{-1}(D)$ from each $X' _b$ in the family $\cX'$ to achieve trivial canonical bundle. 

\begin{lem}\label{gluingmodel}
 We have an isomorphism of the families $(\cY^\circ)^{ur} \cong (\cX^\circ)^{ur}$ over $B^{ur}$ and, in particular, $Y_b^\circ\cong X_b^\circ$ where $Y_b^\circ$ is a member of the family $\cY^\circ$. 
\end{lem}

\begin{proof}

For type $A$, we have a semi-universal $\C^*$-deformation of $A_{n-1}$ singularities (see \cite[Theorem 1]{katz1992gorenstein})  as follows:
\begin{equation}
\begin{aligned}
\sigma': H:=\{xy- s^n - b_2s^{n-2}- ...- b_n = 0\} \subset  \C^3 \times \C^{n-1} &\to \C^{n-1}\cong \ft/W \\ 
(x,y,s,b_2,...,b_n) &\mapsto (b_2,...,b_n)
\end{aligned}
\end{equation}
The map $\sigma'$ is $\C^*$-equivariant if we endow the following $\C^*$-actions on $\C^3$ and $\C^{n-1}$:
\begin{equation}\label{eq:weights}
    (x,y,s)\mapsto (\lambda^2 x, \lambda^{2(n-1)}y,\lambda^2 s) , \quad (b_2,...,b_n)\mapsto (\lambda^4b_2,...,\lambda^{2n}b_n).
\end{equation}
Since the semi-universal $\C^*$-deformation of a simple singularity is unique up to isomorphism, the two deformations $\sigma$ and $\sigma'$ are isomorphic. In other words, the Slodowy slice $S$ contained in $\fg$ is isomorphic to the hypersurface $H$ in $\C^3\times \C^{n-1}$ as semi-universal $\C^*$-deformation. Note that it is important to choose the $\C^*$-action on $\C^{n-1}\cong \ft/W$ and $\C^3$ as above for $S$ and $H$ to be isomorphic as $\C^*$-deformation (see \cite[Remark 2.5.3]{beck2020folding}). 

Next, let's turn to the global situation. We again have the isomorphism of associated bundles
\begin{equation*}
    L|_{\sm^\circ}\times_{\C^*} \C^* \cong  K_{\sm}(D)|_{\sm^\circ}\times_{\C^*} \C^*
\end{equation*}
with the weights of the $\C^*$-action on the left hand side being twice the weights on the right hand side. Hence, the associated bundle $L|_{\sm^\circ}\times _{\C^*} \C^3$ is  
\begin{equation*}
    L^2|_{\sm^\circ}\oplus L^{2(n-1)}|_{\sm^\circ}\oplus L^2|_{\sm^\circ} \cong (K_\sm(D)\oplus K_\sm(D)^{\otimes n-1}\oplus K_\sm(D))|_{\sm^\circ}\cong V|_{\sm^\circ}
\end{equation*}
Also, since the elementary modification is an isomorphism i.e. $ V|_{\sm^\circ}\cong W|_{\sm^\circ}$ away from $D$, the previous construction (\ref{defining equation}) of the family $\pi^\circ:(\cX^\circ)^{ur} \to B^{ur}$ as a family of hypersurfaces in the total space of $W|_{\sm^\circ}$  is equivalent to the construction as the pullback of the gluing of $H$ and $\sigma'$ over $K_\sm (D)|_{\sm^\circ}$: 
\begin{equation}\label{eq:Slodowygluing}
    \begin{tikzcd}
    (\cX^\circ)^{ur} \arrow[r] \arrow[d, "\pi^\circ"] & \bm{H}|_{\sm^\circ} \subset \Tot(K_\sm(D)|_{\sm^\circ}\times_{\C^*} \C^3) \times \Tot(K_\sm(D)|_{\sm^\circ}\times_{\C^*} \ft/W )\arrow[d,"\bm{(\sigma')}|_{\sm^\circ}"] \\
    \Sigma^\circ \times B^{ur} \arrow[r, "ev"] & \bm{U}|_{\sm^\circ} =\Tot(K_\Sigma(D)|_{\Sigma^\circ} \times_{\C^*} \ft/W) 
    \end{tikzcd}
\end{equation}
where we define $\bm{\sigma'}:\bm{H} = \Tot(K_\sm(D)\times_{\C^*} H)\to \bm{U}$ and all the $\C^*$-actions in the diagram are understood as having half the weights in (\ref{eq:weights}). By the argument that $S$ and $H$ are isomorphic as $\C^*$-deformation, we have that $\bm{\sigma}|_{\sm^\circ}:\bm{S}|_{\sm^\circ}= \Tot(L|_{\sm^\circ}\times_{\C^*} S)  \to \bm{U}|_{\sm^\circ}$ and $\bm{\sigma'}|_{\sm^\circ}: \bm{H}|_{\sm^\circ}\to \bm{U}|_{\sm^\circ}$ are also isomorphic. By pulling back this isomorphism along the evaluation map to $\sm^\circ \times B^{ur}$, we get the isomorphism $(\cY^\circ)^{ur} \cong (\cX^\circ)^{ur}. $

\end{proof}


\begin{prop}
The relative intermediate Jacobian fibration $\pi^{ur}: \mathcal{J}(\cX ^{ur}/B^{ur}) \to B^{ur}$ is a semi-polarized integrable system. 
\end{prop}
\begin{proof}
By the relation (4.2), it is enough to show that there exists a Seiberg-Witten differential associated to the subfamily $({\cX}^\circ)^{ur} \to B^{ur}$. In other words, we need to construct a holomorphic volume form ${\lambda_{CY}}^\circ$ on $(\cX^\circ)^{ur}$ which yields the nowhere vanishing holomorphic volume form $\lambda^\circ_{CY,b} \in H^0(X_b^\circ, K_{X_b^\circ})$ for each $b \in B^{ur}$ and satisfies the condition (\ref{def:SW condition}).

First, the holomorphic volume form ${\lambda_{CY}}^\circ$ is obtained from the holomorphic 3-form ${\lambda}$ on $\bm{S}$. Note that the Kostant-Kirillov form on $\fg$ induces the nowhere vanishing section in $ \nu \in H^0(S, K_{\sigma})$. One can glue the sections over $L$ by tensoring with local frames in the pullback of $K_\Sigma$, which turns out to be the holomorphic 3-form $\lambda$ on $\bm{S}$ \cite{diaconescu2006intermediate}\cite{beck2017hitchin}. By restricting $\lambda$ to $\Sigma^\circ$, it becomes a global holomorphic 3-form whose pullback to $(\cX^{\circ})^{ur}$ 
is the desired volume form $\lambda_{CY}^\circ \in H^3(X^\circ_b, \C)$. 
Next, the proof that ${\lambda^\circ_{CY}}$ becomes the Seiberg-Witten differential relies on our main result (Theorem \ref{thm:main meromorphic DDP}). In particular, we identify the volume form ${\lambda^\circ_{CY}}$ with the Seiberg-Witten differential for the Hitchin system so that the form  ${\lambda_{CY}^\circ}$ automatically satisfies the condition (\ref{def:SW condition}). Therefore, it follows from Proposition \ref{SWdifferentials and S-PIS} that $\mathcal{J}(\cX ^{ur}/B^{ur}) \to B^{ur}$ is a semi-polarized integrable system. 
\end{proof}
 
